Adaptive Steering Control for Steer-by-Wire Systems

Steer-by-Wire (SBW) systems are being adapted widely in semi-autonomous and fully autonomous vehicles. The main control challenge in a SBW system is to follow the steering commands in the face of parametric uncertainties, external disturbances and actuator delay; crucially, perturbations in inertial parameters and damping forces give rise to state-dependent uncertainties, which cannot be bounded a priori by a constant. However, the state-of-the-art control methods of SBW system rely on a priori bounded uncertainties, and thus, become inapplicable when state-dependent dynamics become unknown. In addition, ensuring tracking accuracy under actuator delay is always a challenging task. This work proposes two control frameworks to overcome these challenges. Firstly, an adaptive controller is proposed to tackle the state-dependent uncertainties and external disturbances in a typical SBW system without any a priori knowledge of their structures and of their bounds. The stability of the closed-loop system is studied analytically via uniformly ultimately bounded notion and the effectiveness of the proposed solution is verified via simulations against the state-of-the-art solution. While this proposed controller handles the uncertainties and external perturbations, it does not consider the actuator delay which sometimes result in decreased accuracy. Therefore, a new adaptive-robust control framework is devised to tackle the same control problem of an SBW system under the influence of time-varying input delay. In comparison to the existing strategies, the proposed framework removes the conservative assumption of a priori bounded uncertainty and, in addition, the Razumikhin theorem based stability analysis allows the proposed scheme to deal with arbitrary variation in input delay. The effectiveness of the both controllers is proved using comparative simulation studies.

==> UpdatesSampleThesisTemplate/LaTex/introduction.tex <==
In this chapter, we first review the existing approaches for control design for steering control in uncertain environments in the backdrop of autonomous driving.  Subsequently, we review the more niche approaches specifically designed for such systems targeting their applications in the autonomous driving and other drive-by-wire systems. 

\section{Controller Design for SBW Systems}

The steer-by-wire systems are inherently uncertain systems. These are second order systems whose dynamics vary with changing road conditions and mechanical parameters. Such systems require the controllers which take into all these perturbations and uncertainties. The controller design for such systems has been extensively studied. 
With the aim of making the steer-by-wire systems as close to traditional steering systems, the operation from the hand-wheel to the front wheel is considered as a tele-operation application. The main issue that we want to tackle here to ensure the tracking control of the steering actuator on the commands recieved from the steering wheel. In the pursuit of this goal, \cite{PID1} designed a controller which used the traditional closed loop PID control. However, these approaches tend to come with the a large inherent overshoot and response delay due to the integral term involved in the control law.  \\ 
Previous approaches were largely model-free. Another paradigm which researchers used was designing the controller on the basis of model information.  In \cite{Paul} Paul Yih introduced a controller which used acceleration, velocity and feed-forward compensation to improve upon the performance of the steer-by-wire controller response. Continuing on a similar controller design, \cite{5272130} used an online parameter estimation scheme to correctly estimate the parameters for the model and improve the controller performance. The system models used in these approaches are second order models and a number of forces and other uncertainties are not modeled. These uncertainties in the model are the root cause of the poor performance of the model-based controllers. Wang \cite{SMC} used Sliding Mode Controller to handle the model uncertainties. By, considering the rack force as uncertainty, different model based controllers were applied to improve the robustness of the algorithms. \cite{ATC} models the rack force using disturbance observers  

\subsection{Tackling the Uncertainties}

For steering control of the SBW systems, the main challenge is to handle the unpredictable disturbances in the systems. These disturbances include the un-modelled - friction, external rack force and other uncertainties in the model parameters. To tackle uncertainties in SBW systems, researchers have primarily applied robust control \cite{wang2014robust, wang2013sliding} and adaptive control methods \cite{ATC, kim2020adaptive, cetin2012adaptive, zhang2020adaptive, sun2015robust}. While the adaptive control solutions do not require a priori knowledge of the bound of uncertainties compared to a robust controller, a few observations worth mentioning: the state-of-the-art adaptive control methods either require structural knowledge of uncertainty \cite{cetin2012adaptive, sun2015robust}, or assume the uncertain dynamics to be bounded by a constant a priori \cite{ATC, kim2020adaptive, zhang2020adaptive}. However, the upper bound of uncertain dynamics of a SBW system has explicit dependency on states \cite{cetin2012adaptive}; under such an uncertainty setting, presumption of constant upper bound on uncertainty is not only conservative \cite{roy2019overcoming, roy2019simultaneous, roy2019, rodrigues2018global, roy2020towards, roy2018new}, it may even lead to instability \cite{cst_new, roy2020adaptive}.  \\ 

Many of these papers use the assumption that the uncertainty is upper bounded by a constant, but this type of assumption proves to be wrong when the uncertainty has explicit dependency on states, this restricts the state to be upper bounded a priori, and then stability analysis holds no meaning. The proposed approaches assume no such restriction on uncertainty for the problem which is able to outperform all the previous approaches without explicitly modelling the uncertainties and very little prior knowledge of system. 

\section{Controller Design for Time-Delay Systems}
\par Amongst the earliest controllers that were developed for linear time delay systems, a few notable works  include Smith predictor based approach \cite{Ref:6}, Artstein model reduction \cite{Ref:7}, finite spectrum assignment \cite{Ref:8}. Thereafter, the predictor based methodology was extensively investigated by many researchers in \cite{Ref:8, Ref:9, Ref:10, Ref:11, Ref:12, Ref:13, Ref:19, Ref:27}. A stabilizing controller for linear systems with state delay and neutral type delay is reported in \cite{Ref:43} with predefined uncertainty bound. Sampled data control is utilized in \cite{Ref:46-1, Ref:47} for input delay compensation considering known system uncertainty.
The case of feedforward linear systems under both state and input delay is reported by \cite{Ref:14}. Therein, the unknown time delay is predicted adaptively via a projection function, but without considering plant uncertainties. An adaptive control solution for linear systems with linearly parametrized uncertainty with known bounds is reported in \cite{Ref:16}. Adaptive and robust control techniques are utilized in \cite{Ref:17, Ref:29, Ref:30} for linear systems to address the effects of time delay as well as uncertainties. Adaptive backstepping method is used in \cite{Ref:17} for robust stabilization problem of linear non-minimum phase systems subjected to unknown dynamics and input delay. Integral sliding mode control is used by \cite{Ref:29} for uncertain linear systems under time varying delay at the input. However, this scheme relies on a priori known bounds of uncertainties and only suitable for slowly varying input delay. On the other hand, the situation of unknown upper bounds of uncertainty is tackled in \cite{Ref:30} via adaptive sliding mode control. Unfortunately, the adaptation mechanism yields a monotonically increasing switching gain, which might cause high gain instability \cite{roy2017adaptive, ioannou2012robust}. 

\par In comparison, the literature for nonlinear systems with input delay is not vast. Furthermore, the control design for nonlinear systems is more challenging owing to the fact that the closed-loop stability analysis cannot rely on linear boundedness of a system model \cite{Ref:5}. Some earlier works, based on Razumikhin theorem, reported delay dependent \cite{Ref:20} and delay independent \cite{Ref:21} results considering the time delay to be known precisely. A backstepping based predictor approach is proposed by \cite{Ref:24} for delay compensation of forward complete and strict-feedforward nonlinear systems utilizing ODE-PDE cascade transformation. The controller reported in \cite{Ref:41} aims for delay compensation in states and dead zone at the input. However, these control laws cannot handle parametric uncertainties. This issue was addressed in \cite{Ref:31} where a predictor based approach is proposed for constant input delay based on Lyapunov-Krasvoskii method while considering uncertainty in the inertia matrix of Euler-Lagrange systems. The same approach was later extended for time varying input delay in \cite{Ref:32} and also for state delay \cite{Ref:33}. However, the works in \cite{Ref:31, Ref:32, Ref:33} require exact knowledge of input delay and can only negotiate slowly varying input delay. A robust controller is proposed in \cite{roy2017robust} to tackle time varying input delay via Razumikhin theorem based analysis. However, a priori knowledge of uncertainty bounds is required to design any robust controller, which is not always available in practice due to unmodelled dynamics and unknown disturbances. 

\par To handle the situation of unknwon uncertainty bound, adaptive-robust control laws are developed (cf. \cite{Ref:ut, roy2017adaptive, Ref:self, roy2020adaptive, roy2018adaptive, roy2017adaptive2, roy2017adaptive4} and references therein). To compensate time varying network delays in uncertain complex network systems, adaptive sliding mode based control law is developed in \cite{Ref:44}. In a different application, \cite{Ref:45} used adaptive law to evaluate the coupling strength for synchronization of chaotic systems under network induced delay. However, the adaptive laws propsed in \cite{Ref:44, Ref:45} create overestimation of switching gains by not allowing these gains to decrease \cite{roy2019overcoming}. The issue of over- and under-estimation problems of switching gain for uncertain Euler-Lagrange systems under arbitrarily varying input delay was first addressed in \cite{Ref:self}. On the other hand, this work considers the uncertainties to be bounded by an unknown constant, which is a conservative assumption \cite{Ref:ut} when system states are involved in the upper bound structure of uncertainty (cf. \cite{roy2019overcoming, roy2019simultaneous, roy2019new, roy2020adaptive, roy2019auto}). 


